DeSplat: Decomposed Gaussian Splatting for Distractor-Free Rendering

Gaussian splatting enables fast novel view synthesis in static 3D environments. However, reconstructing real-world environments remains challenging as distractors or occluders break the multi-view consistency assumption required for accurate 3D reconstruction. Most existing methods rely on external semantic information from pre-trained models, introducing additional computational overhead as pre-processing steps or during optimization. In this work, we propose a novel method, DeSplat, that directly separates distractors and static scene elements purely based on volume rendering of Gaussian primitives. We initialize Gaussians within each camera view for reconstructing the view-specific distractors to separately model the static 3D scene and distractors in the alpha compositing stages. DeSplat yields an explicit scene separation of static elements and distractors, achieving comparable results to prior distractor-free approaches without sacrificing rendering speed. We demonstrate DeSplat's effectiveness on three benchmark data sets for distractor-free novel view synthesis. See the project website at https://aaltoml.github.io/desplat/.

==> figs/robustnerf.tex <==

\begin{figure*}[ht!]
    \centering
    \setlength{\figurewidth}{0.16\textwidth}
    %\setlength{\figureheight}{.08\textheight}
    \begin{tikzpicture}[
        image/.style = {inner sep=0pt, outer sep=1pt, minimum width=\figurewidth, anchor=north west, text width=\figurewidth}, 
        node distance = 1pt and 1pt, every node/.style={font= {\tiny}}, 
        label/.style = {font={\footnotesize\bf\vphantom{p}},anchor=south,inner sep=0pt}, 
        spy using outlines={rectangle, magnification=2, size=0.485\figurewidth}
        ] 

        %% Row 1 Crab 1
        \node [image] (img-00) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab1/eval_img_0034-gt.png}};
        \spy [red,magnification=1.5] on ($(img-00.north) + (0.0\figurewidth,-0.3\figurewidth)$) in node [right] at ($(img-00.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue] on ($(img-00) + (0.09\figurewidth, - 0.35\figurewidth)$) in node [left] at ($(img-00.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        \node [image,right=of img-00,xshift=0.07\figurewidth] (img-01) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab1/eval_img_0034-sf.png}};
        \spy [red,magnification=1.5] on ($(img-01.north) + (0.0\figurewidth,-0.3\figurewidth)$) in node [right] at ($(img-01.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue] on ($(img-01) + (0.09\figurewidth, - 0.35\figurewidth)$) in node [left] at ($(img-01.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);
        %\spy [blue] on ($(img-01) + (0.3\figurewidth, - 0.25\figurewidth)$) in node [right] at ($(img-01.south) - (0,0.68*0.36\figurewidth)$);

        \node [image,right=of img-01,xshift=0.07\figurewidth] (img-02) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab1/eval_img_0034-sfw.png}};
        \spy [red,magnification=1.5] on ($(img-02.north) + (0.0\figurewidth,-0.3\figurewidth)$) in node [right] at ($(img-02.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue] on ($(img-02) + (0.09\figurewidth, - 0.35\figurewidth)$) in node [left] at ($(img-02.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);
        
        \node [image,right=of img-02,xshift=0.07\figurewidth] (img-03) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab1/val_0034.png}};
        \spy [red,magnification=1.5] on ($(img-03.north) + (0.0\figurewidth,-0.3\figurewidth)$) in node [right] at ($(img-03.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue] on ($(img-03) + (0.09\figurewidth, - 0.35\figurewidth)$) in node [left] at ($(img-03.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        \node [image,right=of img-03,xshift=0.07\figurewidth] (img-04) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab1/eval_img_0034-ours.png}};
        \spy [red,magnification=1.5] on ($(img-04.north) + (0.0\figurewidth,-0.3\figurewidth)$) in node [right] at ($(img-04.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue] on ($(img-04) + (0.09\figurewidth, - 0.35\figurewidth)$) in node [left] at ($(img-04.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        %% Row 2 Crab 2
        \node [image, below=0.5\figurewidth of img-00] (img-10) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab2/eval_img_0044-gt.png}};
        \spy [red] on ($(img-10.north) + (-0.22\figurewidth,-0.85\figurewidth)$) in node [right] at ($(img-10.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-10.north) + (0.3\figurewidth, - 0.4\figurewidth)$) in node [left] at ($(img-10.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        \node [image,right=of img-10,xshift=0.07\figurewidth] (img-11) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab2/eval_img_0044-sf.png}};
        \spy [red] on ($(img-11.north) + (-0.22\figurewidth,-0.85\figurewidth)$) in node [right] at ($(img-11.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-11.north) + (0.3\figurewidth, - 0.4\figurewidth)$) in node [left] at ($(img-11.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        \node [image,right=of img-11,xshift=0.07\figurewidth] (img-12) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab2/eval_img_0044-sfw.png}};
        \spy [red] on ($(img-12.north) + (-0.22\figurewidth,-0.85\figurewidth)$) in node [right] at ($(img-12.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-12.north) + (0.3\figurewidth, - 0.4\figurewidth)$) in node [left] at ($(img-12.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);
        
        \node [image,right=of img-12,xshift=0.07\figurewidth] (img-13) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab2/val_0041.png}};
        \spy [red] on ($(img-13.north) + (-0.22\figurewidth,-0.85\figurewidth)$) in node [right] at ($(img-13.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-13.north) + (0.3\figurewidth, - 0.4\figurewidth)$) in node [left] at ($(img-13.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        \node [image,right=of img-13,xshift=0.07\figurewidth] (img-14) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/crab2/eval_img_0044-ours.png}};
        \spy [red] on ($(img-14.north) + (-0.22\figurewidth,-0.85\figurewidth)$) in node [right] at ($(img-14.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-14.north) + (0.3\figurewidth, - 0.4\figurewidth)$) in node [left] at ($(img-14.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        % Row 3 Yoda
        \node [image, below=0.5\figurewidth of img-10] (img-20) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/yoda/eval_img_0045-gt.png}};
        \spy [red,magnification=2] on ($(img-20.north) + (-0.22\figurewidth,-0.88\figurewidth)$) in node [right] at ($(img-20.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-20.north) + (-0.17\figurewidth, - 0.2\figurewidth)$) in node [left] at ($(img-20.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        \node [image,right=of img-20,xshift=0.07\figurewidth] (img-21) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/yoda/eval_img_0045-sf.png}};
        \spy [red,magnification=2] on ($(img-21.north) + (-0.22\figurewidth,-0.88\figurewidth)$) in node [right] at ($(img-21.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-21.north) + (-0.17\figurewidth, - 0.2\figurewidth)$) in node [left] at ($(img-21.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        \node [image,right=of img-21,xshift=0.07\figurewidth] (img-22) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/yoda/eval_img_0045-sfw.png}};
        \spy [red,magnification=2] on ($(img-22.north) + (-0.22\figurewidth,-0.88\figurewidth)$) in node [right] at ($(img-22.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-22.north) + (-0.17\figurewidth, - 0.2\figurewidth)$) in node [left] at ($(img-22.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);
        
        \node [image,right=of img-22,xshift=0.07\figurewidth] (img-23) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/yoda/val_0054.png}};
        \spy [red,magnification=2] on ($(img-23.north) + (-0.22\figurewidth,-0.88\figurewidth)$) in node [right] at ($(img-23.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-23.north) + (-0.17\figurewidth, - 0.2\figurewidth)$) in node [left] at ($(img-23.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);

        \node [image,right=of img-23,xshift=0.07\figurewidth] (img-24) {\includegraphics[width=\figurewidth]{images/qualitative/proposal 2/yoda/eval_img_0045-ours.png}};
        \spy [red,magnification=2] on ($(img-24.north) + (-0.22\figurewidth,-0.88\figurewidth)$) in node [right] at ($(img-24.south) + (0.01\figurewidth,-0.68*0.36\figurewidth)$); 
        \spy [blue,magnification=1.5] on ($(img-24.north) + (-0.17\figurewidth, - 0.2\figurewidth)$) in node [left] at ($(img-24.south) - (0.01\figurewidth,0.68*0.36\figurewidth)$);
        
        % labels
        \node[label] (label1) at (img-00.north) {Ground Truth};
        \node[label] (label2) at (img-01.north) {Splatfacto};
        \node[label] (label3) at (img-02.north) {Splatfacto-W-T \cite{xu2024splatfactow}};
        \node[label] (label4) at (img-03.north) {SpotlessSplats \cite{sabour2024spotlesssplats}};
        \node[label] (label5) at (img-04.north) {\ours (ours)};

        % scene labels
        \node[label,rotate=90] (scene1) at (img-00.west) {\itshape Crab (1)};
        \node[label,rotate=90] (scene2) at (img-10.west) {\itshape Crab (2)};
        \node[label,rotate=90] (scene3) at (img-20.west) {\itshape Yoda };
    \end{tikzpicture}
    \caption{\textbf{Additional qualitative results on the RobustNeRF data set \cite{sabour2023robustnerf}.} In the {\it Crab~(1)}, \textit{Crab~(2)} and {\it Statue} scenes, \ours reconstructs static objects and backgrounds accurately. 
    %More qualitative examples in \cref{fig:qualitative-robustnerf-all} in the Appendix.
    %our method generates fewer artifacts compared to the baselines. 
    }
    \label{fig:qualitative-robustnerf-all}
\end{figure*}

==> sec/0_abstract.tex <==
\begin{abstract}
Gaussian Splatting, an explicit representation technique, enables faster image generation in constrained 3D environments with static scenes. However, reconstructing dynamic, real-world environments with distractors remains challenging. Most existing methods for unconstrained novel view synthesis rely on semantic information from foundation models, which introduces additional computational overhead. In this work, we propose a novel method that separates occluders purely based on the inherent properties of Gaussians. Our approach reduces computational costs while achieving comparable results.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Para. 1: NVS and 3D Reconstruction\\

Para.2: NeRF and Gaussian Splatting\\

Para.3: NVS in unconstrained environment\\

Para. 4: Issues of the above mentioned methods\\

Para. 5: Our contributions\\

==> sec/2_related_work.tex <==
\section{Related Work}

\subsection{Semantic Understanding in 3D Gaussian Splatting}
Recently, some works have combined Gaussian Splatting with semantic understanding, enabling applications such as image editing, object removal, and manipulation. For instance, Gaussian Grouping \cite{gaussian_grouping} introduced identity encoding to Gaussians. The identity encoding is regularized by 2D cross-entropy loss and 3D KL divergence loss. They combined the 2D foundation model of SAM \cite{kirillov2023segany} and video tractor DEVA \cite{cheng2023tracking} to mask objects. Similarly, Feature-3DGS \cite{zhou2024feature} introduced feature encoding to Gaussians with the help of LSeg \cite{li2022languagedriven} and SAM \cite{kirillov2023segany}, using teacher-student supervision. In this method, the RGB image and feature map are independently rasterized to preserve per-pixel accuracy. EgoLifter \cite{gu2024egolifter} also used the SAM \cite{kirillov2023segany} to generate segmentation masks, leveraging contrastive learning.

\subsection{Robustness in NeRF}

In the original NeRF, it is assumed that the world is geometrically, materially, and photometrically static, with constant illumination, weather, and layout. However, in real-world scenes, this assumption is often violated due to varying light conditions and transient occluders.

To address this issue, Urban Radiance Field  NeRF in the Wild \cite{martinbrualla2020nerfw} introduced per-image appearance embeddings that are useful for images captured under widely varying lighting and atmospheric conditions. These embeddings facilitate interpolation, mimicking the environment under different illuminations. To filter out occluders, \cite{martinbrualla2020nerfw} separates the scene into "static" and "dynamic" parts using an additional transient MLP head, which predicts density and uncertainty.

RobustNeRF \cite{Sabour_2023_CVPR} introduced a kernel function as a robust estimator, training it as a form of iteratively re-weighted least squares. Unlike NeRF-W, RobustNeRF does not require preprocessing with a pre-trained model. However, both NeRF-W and RobustNeRF rely on photometric loss between two RGB images, making it difficult to separate distractors with similar backgrounds.

Both NeRF-W and RobustNeRF are heuristic algorithms that do not require prior knowledge. However, their heuristic loss functions have room for improvement. For example, NeRF-W may produce foggy residuals, while RobustNeRF can filter out high-frequency static objects along with distractors.

NeRF-HuGS \cite{chen2024nerfhugs} combines the strengths of both heuristic methods and segmentation models. With the help of SAM and heuristics, it can generate clear boundaries for occlusions. It also combines SfM-based heuristics and color-residual heuristics to accurately identify static objects with high-frequency texture patterns and detect high-frequency static objects.

Recently, with the flourish of the multi-modal model, NeRF-on-the-go \cite{ren2024nerf} was introduced to reconstruct scenes from randomly taken photos with varying levels of occlusion. This method requires the foundation model DINOv2 along with a shallow MLP to estimate uncertainty and filter out distractors. It decouples the SSIM loss into luminance, contrast, and structure similarities, which helps separate distractors from backgrounds with similar colors. Additionally, it uses a dilated sampling method, sampling rays from a dilated patch to save memory and improve distractor removal. However, while effective for large occluders such as buses and pedestrians, it struggles with fine distractors due to the down-sampling of the DINO model.


\subsection{Robustness in 3DGS}

Gaussian-W \cite{zhang2024gaussian} first generates feature maps via a U-Net model with ResNet and uses an adaptive sampling method to generate dynamic appearance features. These dynamic and intrinsic features are then fused to decode the color of Gaussians for rasterization. A visibility map created with the pre-trained U-Net is used to filter out potential distractors.

SWAG \cite{dahmani2024swagsplattingwildimages} combines image-dependent appearance encoding, an MLP, and hash encoding to adapt 3D Gaussian Splatting (3DGS) to in-the-wild datasets. To separate static and dynamic parts, SWAG utilizes a Binary Concrete random variable \cite{maddison2017concretedistributioncontinuousrelaxation} to modify the opacity, demonstrating effectiveness in removing distractors.

SpotlessSplats \cite{sabourgoli2024spotlesssplats} pre-computes semantic features using Stable Diffusion \cite{zhang2023tale} and then designs both spatial and spatio-temporal clustering methods to generate inlier/outlier maps. SpotlessSplats also applies appearance encoding that encodes the spherical harmonics (SH) coefficients onto the latent vector.

Wild-GS \cite{xu2024wildgsrealtimenovelview} extracts a global embedding and a visibility map using a U-Net. It also extracts a local embedding from a triplane via U-Net. Depth Anything is used to generate a depth map for projecting to the triplane. The intrinsic feature of each Gaussian, which represents the inherent attributes of the material for each Gaussian, is also learned by this framework. Finally, the global, local, and intrinsic feature embeddings are fused to generate a synthesized spherical harmonics function for rasterization.

WildGaussians \cite{kulhanek2024wildgaussians} uses trainable appearance embedding parameters for both images and Gaussian points via an MLP and feeds the corrected color into the rasterizer. Similar to Nerf-on-the-go \cite{ren2024nerf}, it also utilizes the DINO feature. However, it upsamples the DINO features of predicted and ground truth images and computes their cosine similarity to predict uncertainty. The uncertainty is then turned into a per-pixel binary mask to filter the color for supervision. Sky Handling is also worth mentioning because it uses a Fibonacci sphere sampling algorithm to sample points on a sphere around the scene as part of the initialization.

Splatfacto-W \cite{xu2024splatfactownerfstudioimplementationgaussian} 

\subsection{Robustness in Appearance}
The outside changing light and weather introduce variance of the image, while the camera itself may also automatically adjust the white balance or brightness, to make the photos more suitable for our visuality. To tackle the changing appearance, NeRF-W \cite{martinbrualla2020nerfw} got inspiration from Generative Latent Optimization (GLO) \cite{bojanowski2019optimizinglatentspacegenerative} that introduced per-image appearance embeddings and multilayer perception, to predict the  Urban Radiance Field \cite{}


\subsection{3D Scene Understanding / Scene Composition}

\cite{zhou2024hugs}, \cite{tonderski2024neurad}


Note: GaussianImage?

Below is a summary of the main differences between the GaussianImage \cite{zhang2024gaussianimage} method from the paper and 3D Gaussian Splatting:\\

\begin{itemize} 
\item They simplified the parameters: The 2D Gaussian points only have a position (2D), 2D covariance (3 parameters after decomposition), and color coefficients (3D). As a result, the rasterization process is much faster than with 3D Gaussian Splatting. 
\item They proposed a new rasterization method: The color is obtained using the formula $C_i = \sum c_n * \exp(- \sigma_n)$. Please refer to Eq.7 in the Gaussian Image paper for more details. 
\item They discarded density control since 2D images don't have empty space (i.e., areas with alpha=0). However, we should retain this function because we want to mask occlusions while keeping other areas transparent. 
\end{itemize}

==> sec/3_method.tex <==
\section{Method}


\subsection{Background: 3D Gaussian Splatting}
\label{sec:background}

3D Gaussian Splatting \cite{kerbl20233d} is a novel view synthesis method that utilizes explicit representations of Gaussian points.\\

\textbf{Definition of Gaussian Point.}
Each Gaussian point can be defined as:
\begin{equation}
S_{\Theta_i} = \{p_i, s_i, q_i, \alpha_i, c_i\}
\end{equation}
where $p_i = {x, y, z} \in \mathbb{R}^3$ represents the spatial coordinates of the centroid, $s_i \in \mathbb{R}^3$ denotes the 3D size in standard deviations, $q_i \in \mathbb{R}^4$ is a rotational quaternion, $\alpha_i \in \mathbb{R}$ is an opacity value, and $c_i$ is a color vector represented by spherical harmonics (SH) coefficients.\\
Each Gaussian is described by the function:
\begin{equation}
G(x) = e^{-\frac{1}{2} x^T \Sigma^{-1} x}
\end{equation}
When rendering 2D images, the covariance matrix $\Sigma'$ in camera coordinates is transformed as:
\begin{equation}
\Sigma' = JW\Sigma W^T J^T
\end{equation}
where $J$ is the Jacobian of the projective transformation and $W$ is the viewing transformation.\\
\textbf{Optimization and Densification.}
During optimization, the covariance matrix $\Sigma$ is decomposed as:
\begin{equation}
\Sigma = RSS^T R^T
\end{equation}
Here, $S$ is a scaling matrix and $R$ is a rotation matrix, corresponding to the 3D vector $s$ and quaternion $q$, respectively. These components can be independently optimized.\\

\textbf{Adaptive Control of Gaussians.}
The initial input from Structure-from-Motion (SfM) points is sparse. However, with adaptive control of the Gaussians, the point cloud is densified, and some Gaussians are removed to refine the shape. Specifically, this involves cloning small Gaussians in under-reconstructed regions and splitting large Gaussians in over-reconstructed regions. Techniques such as $\alpha$-reset are employed to manage the Gaussians more effectively.\\

\textbf{Loss Function.}
The optimization is based on the rendering of 2D projections and ground truth images, using the loss function:
\begin{equation}
L = (1 - \lambda) L_1 + \lambda L_{D-SSIM}
\end{equation}

\textbf{Rasterization.}
The rasterizer is designed for fast rendering and sorting to enable approximate $\alpha$-blending. It is implemented with custom CUDA kernels, dividing images into tiles and considering only the Gaussians until $\alpha$ reaches 1.

\subsection{Separation of dynamic and static Gaussians}\\
\\label{proposal1}
The core idea of our method is to separate the occluders from static objects using a set of transient Gaussian points. In this approach, we define two sets of Gaussian points: static Gaussians represent static objects, such as furniture and architecture, while dynamic Gaussians capture the representation of occluders. During training, as the images include occluders, we rasterize both static and dynamic Gaussian points. However, in the evaluation stage, only the static Gaussians are rasterized. In Section~\ref{proposal1}, we discuss the implementation of the separation of dynamic and static Gaussians, along with the associated challenges. In Section~\ref{proposal2}, we detail the methods for combining 2D masks and 3D Gaussians, and in Section~[xxx], we explain appearance modeling and background processing.

\textbf{Initialization.} For the initialization of static Gaussians, we follow the method in \cite{kerbl20233d}, where the means are extracted from the COLMAP point cloud. For transient Gaussians, we randomly place a set of Gaussians densely in front of each camera.

\textbf{Densification.} Both static and transient Gaussians coexist within the 3D space, and their behavior in terms of adaptive density control follows the same principles as in 3D Gaussian Splatting \cite{kerbl20233d}.

\textbf{Removal of Invisible Gaussians.} During the optimization process, some points may move and rescale, causing them to fall outside the frame in certain views. For static Gaussians, they may still be visible in other views, allowing them to be optimized further. However, dynamic Gaussians are intended to be visible only in a specific image. If they become invisible, they can no longer be optimized in subsequent steps and will remain outside the frame. To address this, we track the maximum radius of each dynamic Gaussian point when the corresponding frames are optimized. If the radius value is zero, it indicates the dynamic Gaussian is invisible in that frame. If a point has a zero radius across all frames, we consider it to be outside the frame and remove it.

However, some points might initially have a high radius value but move out of the frame while still retaining that value. To prevent this, we reset the maximum radius value to zero at regular intervals, similar to the opacity reset.

\textbf{Optimization.} The dynamic Gaussians share the same learning rate as the static Gaussians. We use the $L_1$ loss and SSIM loss, configured identically to those in 3D Gaussian Splatting \cite{kerbl20233d}, to learn the properties of the Gaussians.

To bring the dynamic Gaussian points as close to the camera as possible, we apply depth regularization. During the training process, since both dynamic and static points are visible, if the dynamic points attempt to explain the static Gaussians, it can cause the static points to become sparse and incomplete. Depth regularization helps prevent this by encouraging dynamic Gaussians to stay near the camera.

The final loss function is: 
$$\mathcal{L} = \mathcal{L}_{color} + \lambda_{depth}\mathcal{L}_{depth}$$
where
$$\mathcal{L}_{color} = \lambda_1 \mathcal{L}_{L1} + (1-\lambda_1) \mathcal{L}_{SSIM}$$
$$\mathcal{L}_{depth} = \sum_{i=0}^{N}\text{depth} \text{ for } \alpha>0$$

Here, $N$ denotes the number of cluttered images, and $\text{depth}_i$ represents the average depth of the dynamic Gaussian points relative to the camera in image $i$.

\textbf{Implementation.} For our experiments, we set $\lambda_{\text{depth}}$ to 20 and the number of initial dynamic Gaussians per image to 500.

\textbf{Confusion in Different Views.} This approach assumes that the Gaussian points in front of the camera are only visible in that specific view. In scenes where the dynamic Gaussians for one image are only visible to a specific camera and invisible to all other cameras, this method works well, as in the "Yoda" scene. However, in the "Patio" and "Statue" scenes, the camera views overlap. As a result, the dynamic Gaussians from one view may cause confusion in another view.

To address these issues, per-image identity can be useful. We can control whether points are visible in certain views. Inspired by GaussianImage \cite{zhang2024gaussianimage}, we replace the dynamic Gaussians with 2D masks.

\subsection{Replacing Dynamic Gaussians with 2D Masks}
\label{proposal2}

Gaussian Splatting can not only be used for novel view synthesis; it also shows great performance for single-image fitting \cite{zhang2024gaussianimage}. In this approach, we aim to learn the masks of dynamic objects via image-specific dynamic Gaussians. The dynamic Gaussians and static Gaussians no longer share the same space.

In the entire training pipeline, we have a \textbf{3D scene} for the static objects and many parallel 3D scenes that serve as 2D masks (referred to as the \textbf{2D masks} below). We have only one 3D scene for the static objects, while the number of 2D masks corresponds to the number of images. The \textbf{3D scene} uses the same optimization strategy as in Splatfacto. The \textbf{2D scenes} exist in 3D space but do not coexist with the 3D scene. Each image has its own corresponding 3D space. Using our blending function, the model learns both the 3D scene and the 2D scenes.

\textbf{Initialization.} Ideally, the static part should be shared across all images, while the view-specific Gaussians represent only the transient objects. We store the dynamic points in a dictionary format $\{Gaussians_i\}^N_{i=1}$, where $N$ represents the number of training images. For each training image $i$, there are a certain number of Gaussians with properties such as means, opacities, scales, quaternions, and spherical harmonic (SH) features. During rendering and optimization, we select the properties from the dictionary corresponding to that view and record the gradients independently.

\textbf{Rendering.} We combine transient and static points using $\alpha$-blending. We assign the background as $bg$, the static objects as $3D$, and the transient occluders as $2D$. The formulation is as follows:
First, we combine the static objects and the background:
\[
C_{\text{3D+bg}} = C_{\text{3D}} + (1 - \alpha_{\text{3D}}) \cdot C_{\text{bg}}
\]
Next, we combine the transient occluders with the result:
\[
\begin{aligned}
C_{\text{2D+3D+bg}} &= C_{\text{2D}} + (1 - \alpha_{\text{2D}}) \cdot C_{\text{3D+bg}} \\
&= C_{\text{2D}} + (1 - \alpha_{\text{2D}}) \cdot C_{\text{3D}} + (1 - \alpha_{\text{2D}})(1 - \alpha_{\text{3D}}) \cdot C_{\text{bg}}
\end{aligned}
\]

\textbf{Densification.} Since the occluders vary between images—some having large occluders and others having small ones—we need to use adaptive density control (ADC) to adjust the number of Gaussians. Unlike the ADC in 3D Gaussian Splatting, which records gradients after each step and densifies the Gaussian points every 100 steps, we densify the points representing an image every time the image is seen $t$ times. During the densification process, all behaviors of the 2D mask Gaussian points—including culling, splitting, and duplication—remain the same as in 3D Gaussian Splatting.

\textbf{Regularization.} In some cases, the dynamic Gaussian points may attempt to represent static objects, or the transient mask may try to cover static areas. During the training process, since the per-view Gaussians can fit both static and dynamic objects well, the training loss tends to be low. However, during evaluation, the loss is higher because the static Gaussians are sparse. This issue has been observed in many methods dealing with complex scenes. Some studies address this by adding a regularization term to minimize the overlap as much as possible.

--- To be updated: ---
In our method, we have tried the following method but without a good result:\\
\begin{itemize}
    \item Defining a "masked" area, which denotes the area with occluders. Adding value regularization to the "masked" area.
    \item Adding depth regularization to each rendered 2D Image.
    \item Adding alpha regularization to each 2D image.
\end{itemize}


==> sec/4_experiments.tex <==
\textbf{Datasets.}

\\

\textbf{Baselines.}

\\

\textbf{Metrics.}

\\

\textbf{Implementation details.} For the initialization of dynamic Gaussians, we set the number of dynamic Gaussians per image to 500.

==> sec/5_conclusions.tex <==
\section{Conclusions}
